Large random matrix approach for testing independence of a large number of Gaussian time series

The asymptotic behaviour of Linear Spectral Statistics (LSS) of the smoothed periodogram estimator of the spectral coherency matrix of a complex Gaussian high-dimensional time series $(\y_n)_{n \in \mathbb{Z}}$ with independent components is studied under the asymptotic regime where the sample size $N$ converges towards $+\infty$ while the dimension $M$ of $\y$ and the smoothing span of the estimator grow to infinity at the same rate in such a way that $\frac{M}{N} \rightarrow 0$. It is established that, at each frequency, the estimated spectral coherency matrix is close from the sample covariance matrix of an independent identically $\mathcal{N}_{\mathbb{C}}(0,\I_M)$ distributed sequence, and that its empirical eigenvalue distribution converges towards the Marcenko-Pastur distribution. This allows to conclude that each LSS has a deterministic behaviour that can be evaluated explicitly. Using concentration inequalities, it is shown that the order of magnitude of the supremum over the frequencies of the deviation of each LSS from its deterministic approximation is of the order of $\frac{1}{M} + \frac{\sqrt{M}}{N}+ (\frac{M}{N})^{3}$ where $N$ is the sample size. Numerical simulations supports our results.

==> response-reviewers.tex <==
\section{Answer to the editor}
We thank the editor for his positive evaluation of our paper, and for his advices concerning the revised version. We first mention that we tried to write the paper in a more compact manner. In particular, we skipped a number of intermediate calculations that were not strictly necessary. However, we did not suppress the details of the most technical proofs in order to help the reader. Next, under the advice of Reviewer 1, we used more extensively the Gaussianity of the time series under consideration. This allowed to simplify the evaluation of $\mathbb{E}(\zeta)$ where $\zeta$ is defined by (\ref{eq:def_zeta}), and to avoid the use of the former Lemma 4.3, which, in the Gaussian case, leads to unnecessary tedious calculations. More importantly, the use of Gaussian tools also allowed us to improve significantly the accuracy of our results. The former speed of convergence $\frac{B}{N}$ of our statistics is now the faster rate $u_N$ defined by (\ref{eq:def-uN}), after correction by a $\mathcal{O}\left(\frac{B}{N}\right)^{2}$  deterministic term given in closed from. We also show how to estimate this term so as to keep unchanged the performance of the modified statistics. Although we have omitted certain technical details, the presentation and the proofs of these new results of course make the current version longer than the first submission. Reviewer 1 mentioned other possible simplifications. In particular, Reviewer 1 was not convinced by the importance of the concentration inequalities we developed, which, certainly, make the paper rather technical. However, as explained in our answer to Reviewer 1, we feel that concentration inequalities are mandatory because our statistics is defined as the supremum over the whole frequency interval $[0,1]$ of a certain frequency dependent statistics. In order to evaluate this supremum, it appears necessary to develop exponential concentration results at each frequency, deduce from this concentration for the supremum over finite dense enough frequency grids using the union bound, and finally take benefit of Lipschitz properties to deduce the rate of convergence of the supremum on the whole frequency interval $[0,1]$. We did not precise this point in the first version, but now explain the importance of concentration tools. All in all, we believe that we have deeply revised our paper, and that it is hard to simplify significantly the current version of the paper. Regarding the importance of our results on a statistical point of view, our main contribution is to have identified a $\mathcal{O}\left(\frac{B}{N}\right)^{2}$ deterministic correction to $\frac{1}{M} \Tr f(\hat{\C}(\nu)) - \int f d\mu_{MP}^{(c_N)}$ that allows to obtain a statistics that converges at the faster rate $u_N$. While we have not established a CLT on the supremum over the frequency of the modified statistics, the derivation of these non obvious results represents in our opinion a first necessary step. We also mention that deriving a CLT on the above mentioned supremum seems us rather difficult, and we feel that a paper collecting the results of the present paper as well as a CLT would be very long and quite technical. We finally mention that we found a mistake in the proof of Lemma \ref{lemma:variance-zeta} establishing that $|\zeta - \mathbb{E}(\zeta)| \prec \frac{1}{B}$. The problem is now fixed. 
\section{Answer to reviewer $1$}
We thank the reviewer for his/her careful reading and for his/her constructive remarks that, hopefully, helped us to improve our manuscript. In particular, a more extensive use of the Gaussianity of the time series allowed us to derive more accurate results. We indeed discovered that our previous evaluations of the rate of convergence of $\sup_{\nu} |\frac{1}{M} \Tr f(\hat{\C}(\nu)) - \int f \, d\mu_{MP}^{(c_N)}|$ were too pessimistic. We now establish that $\sup_{\nu} |\psi_N(f,\nu)|$ converges towards $0$ at the faster rate $u_N$ defined by (\ref{eq:def-uN}), where $\psi_N(f,\nu)$ represents $\frac{1}{M} \Tr f(\hat{\C}(\nu)) - \int f \, d\mu_{MP}^{(c_N)}$ corrected by a deterministic $\mathcal{O}\left( \frac{B}{N} \right)^{2}$ term whose closed form expression is provided. We also show how to estimate this correction to produce a statistics $\hat{\psi}_N(f,\nu)$ for which $\sup_{\nu} |\hat{\psi}_N(f,\nu)|$ still converges towards zero at rate $u_N$. In order to derive these improved results, we modified our general strategy, and wrote $\frac{1}{M} \Tr f(\hat{\C}(\nu)) - \int f \, d\mu_{MP}^{(c_N)}$ as in Eq. (\ref{eq:fundamental-decomposition}). In our first approach, the decomposition was different, and the term that limited the speed of 
convergence was $\frac{1}{M} \Tr f(\tilde{\C}(\nu)) - \frac{1}{M} \Tr f(\frac{\X \X^*}{B+1})$, an $\mathcal{O}_P(\frac{B}{N})$ term.  $\frac{1}{M} \Tr f(\tilde{\C}(\nu)) - \frac{1}{M} \Tr f(\frac{\X \X^*}{B+1})$ is now replaced by its mathematical expectation, which, using Gaussian tools, is shown to be  $\mathcal{O}\left( \frac{B}{N} \right)^{2}$. Moreover, extremely long and tedious evaluations allowed us to evaluate explicitly this $\mathcal{O}\left( \frac{B}{N} \right)^{2}$ term, thus leading to the closed form expression of $\mathcal{O}\left( \frac{B}{N} \right)^{2}$ correction of 
$\frac{1}{M} \Tr f(\hat{\C}(\nu)) - \int f \, d\mu_{MP}^{(c_N)}$. 

\begin{itemize}
    \item {\bf Statistical tests.} 
    \begin{itemize} 
    \item We agree with the reviewer that we do not derive the limit distribution of $\sup_{\nu} |\psi_N(f,\nu)|$ and $\sup_{\nu} |\hat{\psi}_N(f,\nu)|$. We however notice that the present paper establishes non trivial results that allows to evaluate the speed of convergence of these two statistics. The derivation of the speed of convergence of $\sup_{\nu} |\psi_N(f,\nu)|$ and $\sup_{\nu} |\hat{\psi}_N(f,\nu)|$ is of course a first necessary step towards the derivation of a CLT. 
    \item The reviewer apparently feels that our approach can be simplified significantly. We tend to disagree with him/her on this point. In particular, our objective is to study the supremum over the frequency $\nu$ of $|\psi_N(f,\nu)|$ and $|\hat{\psi}_N(f,\nu)|$. In order to evaluate the rate of convergence of $\sup_{\nu} |\psi_N(f,\nu)|$ and $\sup_{\nu} |\hat{\psi}_N(f,\nu)|$, the use of concentration inequalities seems to us mandatory. In particular, it appears necessary to develop exponential concentration results at each frequency, deduce from this concentration for the supremum over finite dense enough frequency grids using the union bound, and finally take benefit of Lipschitz properties to deduce the rate of convergence of the supremum on the whole frequency interval $[0,1]$. Probably that we should have emphasized on this point in the first version of the manuscript in order to motivate the derivation of concentration inequalities. 
    \item Establishing a CLT on $\sup_{\nu} |\psi_N(f,\nu)|$ and $\sup_{\nu} |\hat{\psi}_N(f,\nu)|$ does not seem an easy task, and a paper gathering the results of the present submission and such a CLT would probably be extremely long and technical. In particular, proving a CLT for $\psi_N(f,\nu)$ or  $\hat{\psi}_N(f,\nu)$ for each $\nu$, or even a functional CLT, does not lead, to our best knowledge, to a CLT for $\sup_{\nu} |\psi_N(f,\nu)|$ and $\sup_{\nu} |\hat{\psi}_N(f,\nu)|$. The situation would of course have been different if we decided to use the maximum of the above statistics over a finite amount of frequencies. In this context, the derivation of a CLT would need to establish the joint gaussianity of $(\psi_N(f,\nu_1), \ldots, \psi_N(f,\nu_P))^{T}$ where $P$ is the number of frequencies. However, using the supremum over a finite grid could of course decrease the power of the corresponding tests in the presence of alternatives for which $\nu \rightarrow |\psi_N(f,\nu)|$ exhibits "narrow peaks": under $\mathcal{H}_1$, the maximum of $ |\psi_N(f,\nu)|$ over a low density grid could be much lower than its global maximum, thus reducing the power of the test. Studying  $\sup_{\nu} |\psi_N(f,\nu)|$ and $\sup_{\nu} |\hat{\psi}_N(f,\nu)|$ is thus a problem of interest, both on the theoretical and practical point of views. A compromise between the supremum over the whole interval $[0,1]$ and a fixed set of frequencies $\{ \nu_1, \ldots, \nu_P \}$ would be to study the supremum of $|\psi_N(f,\nu)|$ and $|\hat{\psi}_N(f,\nu)|$ on the set of frequencies $\mathcal{G}_N = \{k \frac{B+1}{N}, k=0, \ldots, \frac{N}{B+1} \}$. 
    In this context, some of the tools developed in \cite{loubatonrosuelvallet2021jmva}, in conjunction with the results of the present submission, could be used to establish that  $\sup_{\nu \in \mathcal{G}_N} |\psi_N(f,\nu)|$ and $\sup_{\nu \in \mathcal{G}_N} |\hat{\psi}_N(f,\nu)|$ follow, after recentering and renormalisation, a Gumble distribution. We finally mention that alternative statistics such as $\int |\psi_N(f,\nu)| d\nu$ 
    or $\int |\psi_N(f,\nu)|^{2} d\nu$ would also make sense, and their limit distribution could be derived from a functional CLT on the random process $(\psi_{N}(f,\nu))_{\nu \in [0,1]}$. This is a relevant topic for future research.   
    \end{itemize}
    \item {\bf Normality.} 
    \begin{itemize}
        \item 
    As the reviewer noticed, the fact that $\hat{\C}(\nu)$ is "close" from a matrix $\frac{\X \X^*}{B+1}$ with $\X$ i.i.d. comes from the Gaussianity of the $M$ time series. The important equation is (\ref{equation:representation-etam}) where the $\mathcal{N}_{\Cbb}(0,\I)$ random row vectors $(\x_m)_{m=1, \ldots, M}$ are introduced. In the non Gaussian case, these row vectors would be mutually independent, but we would not have further information on their probability distributions, except that $\mathbb{E}(\x_m^{*} \x_m) = \I_N$. In this context, if $\X = (\x_1^{T}, \ldots, \x_M^{T})^{T}$, the properties of the large random matrix $\frac{\X \X^*}{B+1}$ are not clear. 
    The rows of $\X$ are mutually independent, but this is not enough to be able to derive results on the limit distribution of $\frac{\X \X^*}{B+1}$. For this, a typical assumption such as $\x_m = \z_m \Thetabs_m$ where the components of $\z_m$ are iid and $\Thetabs_m$ is a deterministic matrix would be needed. More advanced assumptions are based on the probability distribution of the vectors $\x_m$ which should be log concave as in the paper "On the Limiting Empirical Measure of the sum of rank one matrices with log-concave distribution",  Studia Math. 195 (2009), 11-29, by Pajor and Pastur. We feel that formulating such assumptions would be artificial. In our opinion, a more promising approach in the non Gaussian case would be to assume that each time series $(y_{m,n})_{n \in \mathbb{Z}}$ is a linear process generated by an i.i.d. non Gaussian sequence, and evaluate the consequence of this hypothesis on the Fourier transforms vector $\omegabs_m = (\xi_{y_m}(\nu - B/2N), \ldots, \xi_{y_m}(\nu + B/2N))^{T}$, on the distribution of vector $\x_m$ and on matrix $\frac{\X \X^*}{B+1}$. This is a topic for future research. 
     \item As mentioned above, we now use more extensively the Gaussianity of the time series, and this allowed to derive our improved results. In particular, the use of the former Lemma 4.3 mentioned by the reviewer was indeed not necessary, and the use of the Poincaré-Nash inequality, valid in the Gaussian case, provides a simpler answer. 
     \end{itemize}
     \item {\bf Title not appropriate.} We agree on this point that the main subject discussed in this paper is the non asymptotic results concerning the eigenvalues of the smoothed periodogram estimator of the coherency matrix, and not the independence testing of a multivariate time series. We modified the title in accordance with this.
     \item {\bf Other benchmarks.} We thank the reviewer for pointing out to our attention the paper by Pan et al. As mentioned in our revised manuscript, this paper proposes a large random matrix approach to test that the $M$ time series are uncorrelated in the regime where $M$ and $N$ are of the same order of magnitude. In our paper, $\frac{M}{N} \rightarrow 0$, and the use of spectral density estimates seems more relevant. However, as both reviewers pointed out, our result does not allow to design a properly defined test statistics which prevents to control the type I error. We thus decided to remove the section about the detection of an alternative and cannot compare in a fair fashion our approach with the proposal of Pan et al. 
\end{itemize}
\section{Answer to reviewer 2}
We thank the reviewer for his/her evaluation of our paper. Here are our answers to his/her 3 remarks.
\begin{itemize}
    \item We have given some sufficient conditions that imply Assumption \ref{assumption:regularity}, and provided examples. 
    \item If $B$ and $N$ are of the same order of magnitude, the results of the paper do not hold anymore. In particular, matrices $\hat{\C}(\nu)$ and $\tilde{\C}(\nu)$ do not behave as 
    a Wishart matrix (see Theorem \ref{theorem:C_approximation_Wishart} and the rate of convergence of the norm of the error between  $\hat{\C}(\nu)$, $\tilde{\C}(\nu)$ and the Wishart matrix). In particular, the property $\frac{1}{M} \Tr f(\hat{\C}(\nu) - \int f d\mu_{MP}^{(c_N)} \rightarrow 0$ does not hold. If $B$ and $N$ are of the same order of magnitude, so are 
    $M$ and $N$, and, as mentioned in the introduction, other tests based on the sample covariance matrix defined by (\ref{eq:def-hatR}) have to be used (see in particular the paper  \cite{pangaoyang2014jasa}). 
    \item We agree with the reviewer that the asymptotic distribution of the Linear Spectral Statistic considered is unknown. For this reason, we decided to remove the subsection related to the behaviour of the LSS under an alternative, and focus only on the results concerning the concentration of the LSS under $\Hcal_0$. 
\end{itemize}
